Real-Time Forward Kinematics and Jacobians for Control of an MRI-Guided Magnetically Actuated Robotic Catheter

This paper presents a forward kinematics and analytical Jacobian computation approach for real-time control of a novel magnetic resonance imaging (MRI)-actuated robotic catheter. The MRI-actuated robotic catheter is modeled as a series of rigid and flexible segments and actuated by magnetic torques generated on a set of current-carrying microcoils embedded on the catheter body by the magnetic field of the MRI scanner. First, a real-time forward kinematic modeling approach of the robotic catheter employing the static Cosserat-rod theory is presented. Second, the analytical calculation approach of the forward kinematic Jacobians of the proposed forward kinematic model is presented. The accuracy, reproducibility, and computational efficiency of the proposed methods are evaluated using a robotic catheter prototype with a single coil set, where catheter tip trajectories collected by a catadioptric stereo camera tracking system are validated using the desired tip trajectories. Experimental results demonstrate that the proposed method can successfully control the catheter in an open loop to perform complex trajectories with real-time computational efficiency, paving the way for accurate closed-loop control with real-time MR-imaging feedback.

==> result.tex <==

\section{Results}\label{section:results}
In this section, the results of parameter estimation using the Cosserat-rod model are reported. The experimental open-loop control performance including reproducibility and accuracy is presented. 

\subsection{Parameter Estimation Results}\label{section:paramest_results}
The robotic catheter used in the experiments has two flexible segments separated by one rigid segment. The lengths of each segment from proximal to distal ends is given as 29 mm, 13 mm, and 104 mm, respectively. The catheter tubing has the inner radius of 0.84 mm and outer radius of 1.33 mm. In the parameter estimation experiments, the catheter was actuated by three sets of currents. Fig.~\ref{fig:param_est_trajectory} shows the catheter trajectories by actuating the axial coil for bending motion, one side coil for twisting motion, and the other side coil which is orthogonal to the previous one for bending motion, respectively. The solid blue and red lines show the estimated deflection motion locations of the catheter body and estimated locations of the actuator on the catheter from the model. The red circles show the actual locations of the catheter tip using the same current sets. The estimations were performed by minimizing the errors of the tip locations between the actual deflection motion and the motion estimated using the model.

Six catheter parameters including Young's modulus, shear modulus, the coil alignment angle on the catheter, the number of winding coil turns and the cross-sectional areas of the actuator, the actuation coil mass, and the catheter density (mass per length), were estimated using the collected data of the mentioned deflection motions. The estimated parameters for the Pebax35 catheter version and the Qosina version are respectively given in Table~\ref{tb:crmparameters_pebax} and~\ref{tb:crmparameters_qosina}.    

\begin{figure*}
\centering
\begin{subfigure}[t]{.32\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/qosina_param_est_axial-backup.jpg}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.32\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/qosina_param_est_axial-coil1.jpg}
  \caption{}
  \label{fig:sfig2}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.32\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/qosina_param_est_axial-coil2.jpg}
  \caption{}
  \label{fig:sfig3}
\end{subfigure}
% \hfill
\caption{Trajectories used for parameter estimations. The solid blue and red lines show the estimated deflection motion locations of the catheter body and estimated locations of the actuator on the catheter from the model. The red circles show the actual locations of the catheter tip. (a) Trajectory of the catheter with the axial coil actuated for bending motion. (b) Trajectory of the catheter with one side coil actuated for twisting motion. (c) Trajectory of the catheter with the other side coil actuated for bending motion.}
\label{fig:param_est_trajectory}
\end{figure*}


\begin{table}[t]
\caption{Estimated parameters using the Cosserat-rod kinematic model of the catheter made of Pebax35 material}
\begin{center}
\begin{tabular}{>{\centering}m{1em} >{\centering}m{1em} *{2}{>{\centering\arraybackslash}m{2cm}}}
\toprule
 \multicolumn{2}{c|}{Model Parameters} & {Estimated Values} \\
\midrule
 \multicolumn{1}{c|}{ Young's Modulus ($MPa$) } &  \multicolumn{1}{c|}{ $E$ }  & 31.03\\
\midrule
 \multicolumn{1}{c|}{ Shear Modulus ($MPa$) } &  \multicolumn{1}{c|}{ $G$ }  & 8.11\\
 \midrule
 \multicolumn{1}{c|}{ Coil Alignment Angle in X and Y axis ($rad$) } &  \multicolumn{1}{c|}{ $\theta_x, \theta_y$ }  & 3.25, 0.06\\
 \midrule
 \multicolumn{1}{c|}{ Turn-Area Matrix  } &  \multicolumn{1}{c|}{$NA$ }  & diag([-0.43, 0.57, 0.71])\\
 \midrule
 \multicolumn{1}{c|}{ Actuation Coil Mass ($g$) } &  \multicolumn{1}{c|}{ $M$ }  & 2.78$\times$$10^{-9}$\\
\midrule
 \multicolumn{1}{c|}{ Mass per length ($g/mm$) } &  \multicolumn{1}{c|}{ $\rho$  }  & 5.89$\times$$10^{-11}$\\
\bottomrule\end{tabular}
\label{tb:crmparameters_pebax}
\end{center}
\vspace{-0.1in}
\end{table}


\begin{table}[t]
\caption{Estimated parameters using the Cosserat-rod kinematic model of the catheter made of Qosina material}
\begin{center}
\begin{tabular}{>{\centering}m{1cm} >{\centering}m{1em} *{2}{>{\centering\arraybackslash}m{2cm}}}
\toprule
 \multicolumn{2}{c|}{Model Parameters} & {Estimated Values} \\
 \midrule
 \multicolumn{1}{c|}{ Young's Modulus ($MPa$) } &  \multicolumn{1}{c|}{ $E$ }  & 14.54\\
\midrule
 \multicolumn{1}{c|}{ Shear Modulus ($MPa$) } &  \multicolumn{1}{c|}{ $G$ }  & 2.82\\
 \midrule
 \multicolumn{1}{c|}{ Coil Alignment Angle in X and Y axis ($rad$) } &  \multicolumn{1}{c|}{ $\theta_x, \theta_y$ }  & -0.20, -0.16\\
 \midrule
 \multicolumn{1}{c|}{ Turn-Area Matrix  } &  \multicolumn{1}{c|}{$NA$ }  & diag([-0.43, 0.54, 0.48])\\
 \midrule
 \multicolumn{1}{c|}{ Actuation Coil Mass ($g$) } &  \multicolumn{1}{c|}{ $M$ }  & 1.64$\times$$10^{-7}$\\
\midrule
 \multicolumn{1}{c|}{ Mass per length ($g/mm$) } &  \multicolumn{1}{c|}{ $\rho$  }  & 3.06$\times$$10^{-9}$\\
\bottomrule\end{tabular}
\label{tb:crmparameters_qosina}
\end{center}
\vspace{-0.1in}
\end{table}


\subsection{Model Performance}\label{section:model_performance}
The proposed model is validated using four distinct trajectories (circle, lemniscate, rectangle, and butterfly). The catheter motions are recorded and tracked by the catadioptric stereo tracking system under the open-loop control. The catheter is actuated by the calculated actuation currents of each trajectory. Fig.~\ref{fig:example_trajectory} shows the open-loop trajectories generated using the Cosserat-rod model. The red diamonds represent the desired tip locations on these trajectories. The blue triangles represent the observed trajectories of the tip location collected using the catadioptric stereo tracking system. The tip location difference is used as a metric for comparing the generated trajectories using the proposed model to the actual collected trajectories. The root-mean-square (rms) of all these differences on each trajectory are used as a quantitative metric for the performance of the proposed model.

Shape reproducibility of the open-loop trajectories is presented as a performance metric. We collect the experimental data of each trajectory 10 times and quantify the trajectory reproducibility using two methods. The experimental observed trajectories are compared with the desired trajectories in the first method. The experimental observed trajectories are compared with a reference trajectory, which is randomly selected from one of the experimental observed trajectories in the second method. The rms error between the shapes of the trajectories is used as the similarity metric in both methods. The trajectories can be transformed without scaling until the minimum of the rms error is found. The trajectory comparison results of the first and the second methods are shown in Fig.~\ref{fig:method1_comparison} and Fig.~\ref{fig:method2_comparison}, respectively. The rms errors calculated corresponding to both methods are presented in Table~\ref{tb:table_reproduce_crm_pebax}.

For evaluation of the accuracy of the open-loop trajectory, the rms errors between the open-loop trajectories generated using the Cosserat-rod model and the observed trajectories of the tip location collected using the catadioptric stereo tracking system are reported in Fig.~\ref{fig:example_trajectory} and Table~\ref{tb:table_accuracy_crm_pebax}.

The results of the rms errors of both reproducibility and accuracy performance indicate that the overall shape of the experimental observed trajectory has very good similarity to the corresponding desired trajectory.  


\begin{figure*}
\centering
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/accuracy_circle.jpg}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/accuracy_lemniscate.jpg}
  \caption{}
  \label{fig:sfig2}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/accuracy_rectangle.jpg}
  \caption{}
  \label{fig:sfig3}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/accuracy_butterfly.jpg}
  \caption{}
  \label{fig:sfig4}
\end{subfigure}
\caption{Open-loop trajectories generated using the Cosserat-rod model. The red diamonds represent the desired tip locations on these trajectories. The blue triangles represent the observed trajectories of the tip location collected using the catadioptric stereo tracking system. The unit in all these plots is mm. (a) Circle trajectory. (b) Lemniscate trajectory. (c) Rectangle trajectory. (d) Butterﬂy trajectory.}
\label{fig:example_trajectory}
\end{figure*}


\begin{figure*}
\centering
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method1_circle.jpg}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method1_lemniscate.jpg}
  \caption{}
  \label{fig:sfig2}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method1_rectangle.jpg}
  \caption{}
  \label{fig:sfig3}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method1_butterfly.jpg}
  \caption{}
  \label{fig:sfig4}
\end{subfigure}
\caption{Trajectory comparisons between the desired trajectory and the experimental observed trajectories. The red diamonds represent the desired trajectories. The blue markers represent the observed tip locations. Each trajectory is collected 10 times. The unit in all these plots is mm. (a) Circle trajectory. (b) Lemniscate trajectory. (c) Rectangle trajectory. (d) Butterﬂy trajectory.}
\label{fig:method1_comparison}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method2_circle.jpg}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method2_lemniscate.jpg}
  \caption{}
  \label{fig:sfig2}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method2_rectangle.jpg}
  \caption{}
  \label{fig:sfig3}
\end{subfigure}
% \hfill
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{pictures/method2_butterfly.jpg}
  \caption{}
  \label{fig:sfig4}
\end{subfigure}
\caption{Trajectory comparisons among the experimental observed trajectories. The black circle markers represent the reference trajectory, which is randomly selected from one of the observed trajectories. The blue markers represent the other observed trajectories of the tip location. Each trajectory is collected 10 times. The unit in all these plots is mm. (a) Circle trajectory. (b) Lemniscate trajectory. (c) Rectangle trajectory. (d) Butterﬂy trajectory.}
\label{fig:method2_comparison}
\end{figure*}


\begin{table*}[t]
\caption{Open-Loop Trajectory Reproducibility Performance}
\label{tb:table_reproduce_crm_pebax}
\begin{center}
\def\arraystretch{1.30}
\begin{tabular}{l c c c c c c c c c}
\hline\hline 
& \multicolumn{4}{c}{Method 1} && \multicolumn{4}{c}{Method 2}\\
\cline{2-5}\cline{7-10}
Trajectory & Circle & Lemniscate & Rectangle & Butterfly && Circle & Lemniscate & Rectangle & Butterfly\\ [0.5ex]
\hline
Mean &  1.81 &  2.29 &  3.35 &  2.72 && 0.83 &  0.64 &  0.44 &  0.59\\
Variance &  0.0064 &  0.0130 &  0.0017 &  0.0013 && 0.0792 &  0.0059 &  0.0003 &  0.0102\\
Trial 01 &  1.98 &  2.56 &  3.24 &  2.82 && - &  - &  - &  -\\
Trial 02 &  1.83 &  2.40 &  3.32 &  2.69 && 0.34 &  0.53 &  0.40 &  0.46\\
Trial 03 &  1.81 &  2.33 &  3.35 &  2.72 && 0.42 &  0.52 &  0.44 &  0.48\\
Trial 04 &  1.77 &  2.31 &  3.36 &  2.70 && 0.86 &  0.58 &  0.46 &  0.60\\
Trial 05 &  1.69 &  2.25 &  3.34 &  2.71 && 0.78 &  0.66 &  0.44 &  0.63\\
Trial 06 &  1.69 &  2.24 &  3.37 &  2.74 && 0.73 &  0.65 &  0.46 &  0.44\\
Trial 07 &  1.82 &  2.24 &  3.36 &  2.71 && 0.99 &  0.72 &  0.43 &  0.65\\
Trial 08 &  1.88 &  2.20 &  3.38 &  2.72 && 1.09 &  0.65 &  0.45 &  0.68\\
Trial 09 &  1.86 &  2.16 &  3.38 &  2.71 && 1.20 &  0.76 &  0.45 &  0.69\\
Trial 10 &  1.79 &  2.18 &  3.39 &  2.70 && 1.09 &  0.69 &  0.42 &  0.71\\ [1.0ex]
\hline\hline
\end{tabular}
\end{center}
\footnotesize{The experimental observed trajectories are compared with the desired trajectories in the first method (method 1). The experimental observed trajectories are compared with a reference trajectory, which is randomly selected from one of the experimental observed trajectories in the second method (method 2). The means and variances are calculated from the rms errors. All units are in millimeter.}
\end{table*}


\begin{table}[t]
\caption{Open-Loop Trajectory Accuracy Performance}
\label{tb:table_accuracy_crm_pebax}
\begin{center}
\def\arraystretch{1.30}
\begin{tabular}{l c c c c}
\hline\hline 
Trajectory & Circle & Lemniscate & Rectangle & Butterfly\\ [0.5ex]
\hline
Mean &  4.34 &  6.49 &  4.60 &  3.66\\
Variance &  0.0581 &  0.0063 &  0.0034 &  0.0668\\
Trial 01 &  4.89 &  6.51 &  4.48 &  3.32\\
Trial 02 &  4.10 &  6.53 &  4.54 &  3.33\\
Trial 03 &  4.03 &  6.39 &  4.56 &  3.46\\
Trial 04 &  4.46 &  6.38 &  4.60 &  3.62\\
Trial 05 &  4.36 &  6.57 &  4.59 &  3.75\\
Trial 06 &  4.07 &  6.52 &  4.63 &  3.47\\
Trial 07 &  4.36 &  6.62 &  4.64 &  3.65\\
Trial 08 &  4.41 &  6.39 &  4.66 &  3.88\\
Trial 09 &  4.48 &  6.54 &  4.66 &  4.00\\
Trial 10 &  4.22 &  6.44 &  4.67 &  4.10\\ [1.0ex]
\hline\hline
\end{tabular}
\end{center}
\footnotesize{The means and variances are calculated from the rms errors. All units are in millimeter.}
\end{table}


\begin{table*}[t]
\caption{Open-Loop Trajectory Reproducibility Performance}
\label{tb:table_reproduce_crm_qosina}
\begin{center}
\def\arraystretch{1.30}
\begin{tabular}{l c c c c c c c c c}
\hline\hline 
& \multicolumn{4}{c}{Method 1} && \multicolumn{4}{c}{Method 2}\\
\cline{2-5}\cline{7-10}
Trajectory & Circle & Lemniscate & Rectangle & Butterfly && Circle & Lemniscate & Rectangle & Butterfly\\ [0.5ex]
\hline
Mean &  2.84 &  5.33 &  5.97 &  6.44 && 0.41 &  0.35 &  0.69 &  0.68\\
Variance &  0.0075 &  0.0016 &  0.0017 &  0.0045 && 0.0114 &  0.0011 &  0.0046 &  0.0988\\
Trial 01 &  2.77 &  5.26 &  5.88 &  6.56 && - &  - &  - &  -\\
Trial 02 &  2.91 &  5.29 &  5.93 &  6.53 && 0.35 &  0.32 &  0.59 &  0.29\\
Trial 03 &  2.77 &  5.27 &  5.95 &  6.43 && 0.25 &  0.31 &  0.64 &  0.87\\
Trial 04 &  2.96 &  5.36 &  5.98 &  6.46 && 0.52 &  0.34 &  0.68 &  0.34\\
Trial 05 &  2.95 &  5.32 &  5.95 &  6.47 && 0.47 &  0.33 &  0.63 &  0.35\\
Trial 06 &  2.80 &  5.35 &  5.97 &  6.44 && 0.27 &  0.40 &  0.63 &  0.40\\
Trial 07 &  2.94 &  5.37 &  5.98 &  6.46 && 0.59 &  0.41 &  0.70 &  0.79\\
Trial 08 &  2.87 &  5.35 &  6.01 &  6.40 && 0.41 &  0.34 &  0.75 &  0.92\\
Trial 09 &  2.74 &  5.35 &  6.02 &  6.38 && 0.38 &  0.34 &  0.77 &  0.91\\
Trial 10 &  2.73 &  5.37 &  6.02 &  6.31 && 0.46 &  0.36 &  0.80 &  1.21\\ [1.0ex]
\hline\hline
\end{tabular}
\end{center}
\footnotesize{The experimental observed trajectories are compared with the desired trajectories in the first method (method 1). The experimental observed trajectories are compared with a reference trajectory, which is randomly selected from one of the experimental observed trajectories in the second method (method 2). The means and variances are calculated from the rms errors. All units are in millimeter.}
\end{table*}

\begin{table}[t]
\caption{Open-Loop Trajectory Accuracy Performance}
\label{tb:table_accuracy_crm_qosina}
\begin{center}
\def\arraystretch{1.30}
\begin{tabular}{l c c c c}
\hline\hline 
Trajectory & Circle & Lemniscate & Rectangle & Butterfly\\ [0.5ex]
\hline
Mean &  17.11 &  18.14 &  20.11 &  14.29\\
Variance &  0.0162 &  0.0066 &  0.0062 &  0.0050\\
Trial 01 &  17.26 &  18.22 &  20.17 &  14.43\\
Trial 02 &  17.20 &  17.95 &  20.20 &  14.38\\
Trial 03 &  17.19 &  18.16 &  20.07 &  14.29\\
Trial 04 &  17.10 &  18.17 &  20.24 &  14.27\\
Trial 05 &  17.24 &  18.18 &  20.05 &  14.29\\
Trial 06 &  16.88 &  18.11 &  20.16 &  14.30\\
Trial 07 &  17.18 &  18.04 &  19.96 &  14.30\\
Trial 08 &  17.15 &  18.21 &  20.14 &  14.21\\
Trial 09 &  17.06 &  18.11 &  20.09 &  14.27\\
Trial 10 &  16.89 &  18.21 &  20.06 &  14.16\\ [1.0ex]
\hline\hline
\end{tabular}
\end{center}
\footnotesize{The means and variances are calculated from the rms errors. All units are in millimeter.}
\end{table}



\begin{table*}[t]
\caption{Open-Loop Trajectory Reproducibility Performance}
\label{tb:table_reproduce_continuum_qosina}
\begin{center}
\def\arraystretch{1.30}
\begin{tabular}{l c c c c c c c c c}
\hline\hline 
& \multicolumn{4}{c}{Method 1} && \multicolumn{4}{c}{Method 2}\\
\cline{2-5}\cline{7-10}
Trajectory & Circle & Lemniscate & Rectangle & Butterfly && Circle & Lemniscate & Rectangle & Butterfly\\ [0.5ex]
\hline
Mean &  2.43 &  4.09 &  4.78 &  7.46 && 0.41 &  0.35 &  0.69 &  0.68\\
Variance &  0.0073 &  0.0010 &  0.0004 &  0.0012 && 0.0114 &  0.0011 &  0.0046 &  0.0988\\
Trial 01 &  2.40 &  4.05 &  4.84 &  7.40 && - &  - &  - &  -\\
Trial 02 &  2.52 &  4.08 &  4.77 &  7.44 && 0.35 &  0.32 &  0.59 &  0.29\\
Trial 03 &  2.38 &  4.03 &  4.76 &  7.48 && 0.25 &  0.31 &  0.64 &  0.87\\
Trial 04 &  2.52 &  4.12 &  4.78 &  7.42 && 0.52 &  0.34 &  0.68 &  0.34\\
Trial 05 &  2.54 &  4.10 &  4.77 &  7.43 && 0.47 &  0.33 &  0.63 &  0.35\\
Trial 06 &  2.40 &  4.12 &  4.79 &  7.45 && 0.27 &  0.40 &  0.63 &  0.40\\
Trial 07 &  2.50 &  4.12 &  4.76 &  7.47 && 0.59 &  0.41 &  0.70 &  0.79\\
Trial 08 &  2.44 &  4.11 &  4.78 &  7.50 && 0.41 &  0.34 &  0.75 &  0.92\\
Trial 09 &  2.29 &  4.10 &  4.78 &  7.50 && 0.38 &  0.34 &  0.77 &  0.91\\
Trial 10 &  2.30 &  4.11 &  4.78 &  7.50 && 0.46 &  0.36 &  0.80 &  1.21\\ [1.0ex]
\hline\hline
\end{tabular}
\end{center}
\footnotesize{The experimental observed trajectories are compared with the desired trajectories in the first method (method 1). The experimental observed trajectories are compared with a reference trajectory, which is randomly selected from one of the experimental observed trajectories in the second method (method 2). The means and variances are calculated from the rms errors. All units are in millimeter.}
\end{table*}

\begin{table}[t]
\caption{Open-Loop Trajectory Accuracy Performance}
\label{tb:table_accuracy_continuum_qosina}
\begin{center}
\def\arraystretch{1.30}
\begin{tabular}{l c c c c}
\hline\hline 
Trajectory & Circle & Lemniscate & Rectangle & Butterfly\\ [0.5ex]
\hline
Mean &  5.93 &  5.83 &  6.53 &  8.45\\
Variance &  0.0465 &  0.0144 &  0.1098 &  0.0017\\
Trial 01 &  6.30 &  6.04 &  7.33 &  8.51\\
Trial 02 &  6.15 &  5.69 &  6.80 &  8.44\\
Trial 03 &  6.07 &  5.87 &  6.47 &  8.40\\
Trial 04 &  5.90 &  5.80 &  6.67 &  8.46\\
Trial 05 &  6.12 &  5.95 &  6.44 &  8.43\\
Trial 06 &  5.70 &  5.80 &  6.61 &  8.45\\
Trial 07 &  5.85 &  5.62 &  6.17 &  8.52\\
Trial 08 &  5.91 &  5.94 &  6.35 &  8.47\\
Trial 09 &  5.72 &  5.76 &  6.25 &  8.44\\
Trial 10 &  5.58 &  5.85 &  6.19 &  8.37\\ [1.0ex]
\hline\hline
\end{tabular}
\end{center}
\footnotesize{The means and variances are calculated from the rms errors. All units are in millimeter.}
\end{table}
